Outline of an Independent Systematic Blackbox Test for ML-based Systems

This article proposes a test procedure that can be used to test ML models and ML-based systems independently of the actual training process. In this way, the typical quality statements such as accuracy and precision of these models and system can be verified independently, taking into account their black box character and the immanent stochastic properties of ML models and their training data. The article presents first results from a set of test experiments and suggest extensions to existing test methods reflecting the stochastic nature of ML models and ML-based systems.

==> ConstructiveProbOntology.tex <==
\section{A constructive approach to probabilisticly extend ontologies}\label{section:ConstrProbExtension}
So far, we have assumed that we have a \textit{probabilistically extended ontology}.
But it is obvious that for a complex ontology it is highly non-trivial to extend it probabilistically.
In this chapter, we present an approach to tackle this task.
First, we present a way to obtain a simplified approximation of the distribution.
We then outline how this approach can be refined.

In this chapter, we use our notation from chapter \ref{section:ProbOntology}.
We look for a probability distribution
\bea
p: \Pi_{i=0}^{n} X_i &\rightarrow & \R^+ \hspace{0.1cm}\mbox{probability distribution} \nonumber\\
(x_{j_0}^0,\dots x_{j_n}^n)& \mapsto & p(x_{j_0}^0,\dots x_{j_n}^n) 
\ea

With Bayes \cite{Dudley.2002} we can paraphrase this to
\bea
p(x_{j_0}^0,\dots x_{j_n}^n) &=& 
p(x_{j_0}^0)\cdot p(x_{j_1}^1|x_{j_0}^0)\cdot p(x_{j_2}^2|x_{j_1}^1,x_{j_0}^0)\cdot \\
&& \hspace{0.1cm}\dots p(x_{j_n}^n|x_{j_{n-1}}^{n-1},\dots x_{j_1}^1,x_{j_0}^0) \hspace*{1cm}(Bayes)\nonumber
\ea
($p(\cdot| \cdot)$ the conditional expectation.)

First, we assume the simplest case, that all classes in the ontology can be assigned the possible properties independently.
For the example in chapter \ref{section:Ontology}, we can choose sex and age independently as a first approximation.
In this simplified case the conditional expectations are trivial,
\be
p(x_{j_k}^k|x_{j_{k-1}}^{k-1},\dots x_{j_1}^1,x_{j_0}^0) = p_{X_k}(x_{j_k}^k),
\ee
and with $p_{X_k}(\cdot), k\in \{0,\dots n\}$ denoting the distributions on the classes, the total distribution is their product measure
\be
p(x_{j_0}^0,\dots x_{j_n}^n) = \Pi_{i=0}^{n} p_{X_i}(x_{j_i}^i).
\ee

In the above example of a person, this means that we need to specify the distributions for age and sex as well as for height.
It is easy to find statistics on the Internet that can be used to define these distributions.
Often, however, such a distribution can be estimated well using the central limit theorem \cite{Dudley.}, e.g. in the case of a person's height.
Height has finite means and variances and is real-valued.  
Therefore, if the sample size is large enough, the sampling distribution for the height and its standardized mean are well approximated by a normal distribution.

Having better models for the underlying probability distributions increases the reliability of our test results, see chapter \ref{section:ExpResults}.
The task is to find a good balance between modeling effort and efficiency.
For example, the age pyramid of women is slightly different from that of men, but for identifying a person in a street scene, this difference should be irrelevant to the ML-based system and can be ignored.

In the first step, we ignore subtle dependencies and look at the marginal distributions, i.e. the distributions for single class instantiations.
In this way the probability to find a female or male person is set uniformly to 0.5.

But specifying the marginal distributions is only half the game.
A person's height correlates with their age; children and teenagers tend to be shorter than adults.
The simple example of the person ontology already shows that the classes usually cannot be instantiated stochastically independently.

In simple terms, we will model that children and teenager are up to 1.65m tall.
These are then simple Boolean boundary constraints as described in our ontology.
Given the age of a person we are looking for the conditional expectation $p(x_{Height}|x_{Age})$, i.e. the distribution of heights of a person whose age we know.

With Bayes, $p(x_{Height},x_{Age}) = p(x_{Height}|x_{Age}) \cdot p_{Age}(x_{Age})$ and the problem can be reformulated.
We are looking for a distribution $p_{X_i,X_j}$ with given marginal distributions $p_{X_i},p_{X_j}$ which represents the logical constraint as formulated in the ontology.
Such a distribution is called coupling of the distributions $p_{X_i},p_{X_j}$, see \cite{Villani.2009}.
The classical transport problem can be formulated in this way (Kantorovich-Rubinstein duality, see \cite{Villani.2009}) and so various approaches have been developed to uniquely define and compute such couplings, \cite{Peyre.}.

For the example of Boolean constraints, we found a simple expression for the distribution on the product space, given the marginals.
An explicit solution is given as follows.
\Ex
Let $\chi_I$ be the characteristic function for a subset $I\subset \mathcal{X}$, i.e. $\chi_I(x_i)\equiv 1$ if $x_i \in I$, otherwise 0, and
$I^c=\mathcal{X}-I$ is the complement of I in $\mathcal{X}$.
Let $p_X(I)$ be the probability of the subset $I\subset \mathcal{X}$ with respect to $p_X$.
Similar notation should apply to $J\subset \mathcal{Y}$.

With these notations and $p_X(I)+ p_Y(J)\leq 1$ it can be shown that

\bea
p_{I\rightarrow J}(x_i,y_j)&:=& p_X(x_i)\cdot p_Y(y_j) \cdot \\
&&( \frac{1}{ p_Y(J)}\cdot \chi_{I}(x_i) \cdot \chi_{J}(y_j) + \frac{1}{1-p_X(I)}\cdot \chi_{I^c}(x_i) \nonumber\\ && + \frac{-p_X(I)}{(1-p_X(I))\cdot p_Y(J)}\cdot \chi_{I^c}(x_i) \cdot \chi_{J}(x_j) ) \nonumber
\ea

\noindent defines a coupling of $p_X,p_Y$ that imposes the logical constraint: 

If a property from $I\subset X$ is selected, then only a property from $J\subset Y$ can be selected.
This formula can be generalized to more complex logical constraints.
\Exa

Using comparable methods, we can model broader functional relationships, such as the tendency for a person to be taller as they age.
This requires listing the property subranges and incorporating a certain order.

For example, consider the age and height of a young person.
Partition the age into increasing intervals, as shown in figure 
ef{fig:OntologyPartitioning}, and do the same for height.
This will help to establish functional dependencies.
The linear correlation between age and height can then be used to formulate a linear relationship.
Domain Specific Languages (DSL) can greatly simplify the descriptions, as we will show in a future paper.
With their help, we can use formulas such as age $\sim$ height or mass $\sim size^3$ to describe linear or higher order dependencies.
We model such functional descriptions by metrics in appropriate abstract spaces, so that solutions to the transport problem \cite{Villani.2009,Peyre.} provide us with appropriately modeled couplings.
Further work on this topic is in progress, see also \cite{ProbExtOnt}.

In addition to modelling different dependencies through appropriate couplings to make a probabilistic extension of an ontology feasible and maintainable, the classes should be designed to be as independent as possible.
Graphical probabilistic modeling, see \cite{Koller.2009}, can be very helpful here.
Let's look at the ODD of all street scenes. 
Then the number of people should be selected before further characterizations of a person are made.
Graphical probabilistic modeling helps to structure the ontology well in order to extend it probabilistically and simplifies the task.

Nevertheless, developing a probabilistically extended ontology is a very complex and time-consuming task.
But it makes transparent how the ODD is structured not only in terms of its potential entities, but also how the different realizations are distributed.
This makes it possible to operationalize what should be representative and balanced!
In particular we get an explicit probabilistic approximation of the target environment, the ODD. 
In most cases, the labeling of the training data is not nearly as finely structured as the partitioning of the ODD.
And, if available, we can sample form training data and manually classify it according to the partition, see chapter \ref{section:TestGen}.
In this way, we can use standard statistical tests (hypothesis and correlation tests,\dots, t-test, $Chi^2-$,Mann-Whitney-U,\dots, \cite{Bijma.2017}) to prove the balance of the training data with respect to a selected subset of partitions.

An analysis of the Bernoulli coefficients $\overline{p}_h$ of partitions also allows us to detect weaknesses in our ML-based system.
In a future work we will describe these ideas in more detail.

\subsection{Ethical points of view}
As described in chapter \ref{section:Ontology}, an ontology always reflects our interests.
This is also true for its probabilistic extension.
For example, if we demand for ethical reasons that skin color should not play a role, this is reformulated as a demand for a uniform distribution on the space of skin colors.
The same is true for age and sex.
This means that the distribution underlying our test case selection must be uniform with respect to these properties.
Conversely, given a \textit{probabilistically extended ontology}, it can be checked for consistency with ethical principles, and testing based on it helps to check them for the system under test.

\subsection{Generation of test data}\label{section:TestGen}
Assuming we have a probabilistically extended ontology, Bayes' formula or a graphical probabilistic model also provides us with an algorithm for generating the necessary test data.
First, we sample the properties of the first class $x_0^0 \in X_0$ according to the marginal distribution $p_{X_0}$.
Then we sample the property subset of the next class $X_1$ according to the conditional distribution $p(x_1^1|x_0^0)$, and so on.
We can drop the independent variables, i.e., if $x_i^1$ are uncorrelated with  $x_j^0$, e.g., sex and age, we get $p(x_1^1|x_0^0)=p(x_1^1)$ and sample according to that marginal distribution.
In this way, we sample for all classes the property subranges as given by the ontology, $(x_{j_0}^0,\dots x_{j_n}^n)$ and according to the distribution $p$.
Such a sample can be viewed as an abstract test case description.

The second step is to convert the abstract test cases into concrete test specifications.  
In other words, we need to obtain test data that matches the abstract description given by the different instantiation choices of the classes in our ontology.
This task is similar to the click work required to provide labeled training data.

The sampling procedure then ensures that the test data is representative and balanced with respect to the defined probability model of the ODD.
A statistical evaluation of the test result could thus independently and significantly verify the quality claims of the developers.



==> SystematicTest.tex <==
\section{A Systematic test process for ML-based systems }\label{section:SystematicTest}
Analogous to the systematic test of embedded systems as outlined in \ref{section:SysTestConvES}, we summarise the various activities that are necessary for testing ML-based systems into one process.

\subsection{Creating a probabilistically extended ontology}
In the systematic testing of embedded systems, classification trees are used to describe the expected input space of a system \cite{GrimmGrocht}. The leaves of the tree then specialise in partial aspects of the input space, for which suitable representatives can be defined and systematically combined to form abstract test cases. For ML-based systems, we use ontologies instead of a classification tree, which allows us to specify our assumptions about the input space of the system.  This is common practize \cite{ASAMOpenSCENARIO,scenic,dissSchuldt,CoreOnt2015,Breitenstein.2020,Bogdoll.01.09.2022,Breitenstein.11.02.2021,Guneshka22,Zipfl.21.04.2023,UlHaq.2019} and closer described in chapter \ref{section:Ontology}.

Besides defining the base classes an their properties, the creation of the ontology in step (\textbf{Develop Ontology}, figure \ref{fig:SystTestProcess}) includes the specification of logical dependencies between properties. Moreover, we recommend to choose statistically independent classes whenever possible and to minimize dependencies between different properties, see chapter \ref{section:ConstrProbExtension}. Furthermore, the ontology should be refined enough to satisfy the uniformity hypothesis: \textit{The probability of a negative test result is independent of the specific instantiations for the classes when the properties are selected from the same partition.}.

In the next step (\textbf{Assign Class Probability Distributions}, figure \ref{fig:SystTestProcess}), probability distributions for the  properties of single classes must be specified. These distributions can be either derived from public available statistical data or needs to be modelled through appropriate approximations. The modeling of dependencies between properties of different classes is difficult (\textbf{Model Prob. Class Dependencies}, figure \ref{fig:SystTestProcess}).
Even though, logical dependencies may already be modelled, functional relationships like: Age and height are linearly correlated, should be furhter specified in this phase. A far-reaching technique here is to enumerate and order the properties and then use functional descriptions as outlined in chapter \ref{section:ConstrProbExtension}.

By combining the class probability distributions and the conditional expectations (couplings) modeled by the (functional) dependency descriptions, we compute the distribution over the partitioning space (\textbf{Compute Class Couplings}, figure \ref{fig:SystTestProcess}).

We will go into more detail in a forthcoming work.

% \begin{figure*}
%    \centering
%    \includegraphics[width=0.5\textwidth]{fig/Process.png}
%    \caption{Systematic Testprocess} \label{fig:SystTestProcess}
% \end{figure*}

\begin{figure}
   \centering
   \includegraphics[width=0.5\textwidth]{fig/Process.png}
   \caption{Systematic Testprocess} \label{fig:SystTestProcess}
\end{figure}

In addition, if testers have access to the training data, they can evaluate the representativeness and balance of the training data using the \textit{probabilistically extended ontology} we presented. For this purpose, random samples can be obtained from the training data and statistical hypothesis tests can be applied to these data to check compliance with the probability model given by the ontology.
Depending on the domain and requirements, various methods (t-test, Mann-Whitney U-test, etc. \cite{Bijma.2017}) can be used as outlined in chapter \ref{section:ConstrProbExtension}.


\subsection{Check statistical quality claims}
The statistical quality requirements can now be checked on the basis of a \textit{probabilistically extend ontology}. In a first step (\textbf{Estimate Sample Sizes}, figure \ref{fig:SystTestProcess}), the number of test cases required to test the test hypothesis must be estimated for the specified key figures and agreed significances. For this purpose, the partitioning given by the ontology, the probabilistic extensions and the associated multinomial probability model are used. For details see chapter \ref{section:StatistObs}.
We apply probabilistic programming techniques to estimate this quantity, see \cite{BMCP2021,BARTHE.b}, and create as many abstract test cases in accordance with the probability model so that the classes, their characterisations and properties are statistically covered.


For each abstract test case, i.e. an appropriate sample of properties for each class, we specify a concrete instantiation of these properties.(\textbf{Specify Concrete Testcases}, figure \ref{fig:SystTestProcess}). In order to be independent of the development, we recommend not to use the training and test data sets used in the course of the training for this instantiation, but to try to use new, previously unused data and data sets. 

Given these newly created test data we apply them to the system under test (SUT) and check how often these tests fail (\textbf{Perform Tests}, figure \ref{fig:SystTestProcess}). The test statistics should confirm the expected key figures up to a controlled deviation. Due to the independence of the test sets of the training process, our measured data can be clearly compared with the key figure specified by the developers (\textbf{Check Test Statistic}, figure \ref{fig:SystTestProcess}).If our measured metrics deviate too far from the proposed metrics, we reject the hypothesis. Otherwise, our results are confirmed.

So far we only tested the feasibility of this procedure on simple models.
We have not used developement independent data as test data, but suitable subsets of the training data.
We defined a simple ontology for the labelings and extended it probabilistically.
Our results confirmed that this procedure allows us to check the statistical quality criteria.

 

